Physics-Embedded Neural Networks: Graph Neural PDE Solvers with Mixed Boundary Conditions

Graph neural network (GNN) is a promising approach to learning and predicting physical phenomena described in boundary value problems, such as partial differential equations (PDEs) with boundary conditions. However, existing models inadequately treat boundary conditions essential for the reliable prediction of such problems. In addition, because of the locally connected nature of GNNs, it is difficult to accurately predict the state after a long time, where interaction between vertices tends to be global. We present our approach termed physics-embedded neural networks that considers boundary conditions and predicts the state after a long time using an implicit method. It is built based on an E(n)-equivariant GNN, resulting in high generalization performance on various shapes. We demonstrate that our model learns flow phenomena in complex shapes and outperforms a well-optimized classical solver and a state-of-the-art machine learning model in speed-accuracy trade-off. Therefore, our model can be a useful standard for realizing reliable, fast, and accurate GNN-based PDE solvers. The code is available at https://github.com/yellowshippo/penn-neurips2022.

==> Makefile <==
# Change NAME accordingly
NAME = penn
# DIFF_REF = bb806e391654b4d70b86c2b9636ee770736353d2

TEX = pdflatex
# TEX = pdflatex -shell-escape -interaction=nonstopmode -file-line-error
DVI = dvipdfmx
PRE =  $(TEX) -ini -job-name="preamble" "&pdflatex preamble.tex\dump"
BIB = bibtex


one: $(NAME).tex
	$(TEX) $(NAME).tex
	open $(NAME).pdf

all: pdf view

pdf: $(NAME).pdf

# diff:
# 	cp iclr2021_conference.bbl iclr2021_conference-diffad0f7d35.bbl
# 	yes | latexdiff-vc -s COLOR --disable-auto-mbox --exclude-textcmd="textit,footnote,section,subsection" --graphics-markup=0 --math-markup=0 --git -r $(DIFF_REF) $(NAME).tex
# 	# yes | latexdiff-vc --append-textcmd=scalebox --git -r $(DIFF_REF) $(NAME).tex
# 	$(TEX) $(NAME)-diff$(DIFF_REF).tex
# 	open $(NAME)-diff$(DIFF_REF).pdf

view:
	open $(NAME).pdf

clean:
	$(RM) $(NAME).pdf $(NAME).dvi $(NAME).aux $(NAME).log

$(NAME).pdf: $(NAME).tex
	$(TEX) $(NAME).tex
	bibtex $(NAME)
	$(TEX) $(NAME).tex
	$(TEX) $(NAME).tex
	$(TEX) $(NAME).tex

figure: figure.tex
	$(TEX) figure.tex
	open figure.pdf

